TrojanPuzzle: Covertly Poisoning Code-Suggestion Models

With tools like GitHub Copilot, automatic code suggestion is no longer a dream in software engineering. These tools, based on large language models, are typically trained on massive corpora of code mined from unvetted public sources. As a result, these models are susceptible to data poisoning attacks where an adversary manipulates the model's training by injecting malicious data. Poisoning attacks could be designed to influence the model's suggestions at run time for chosen contexts, such as inducing the model into suggesting insecure code payloads. To achieve this, prior attacks explicitly inject the insecure code payload into the training data, making the poison data detectable by static analysis tools that can remove such malicious data from the training set. In this work, we demonstrate two novel attacks, COVERT and TROJANPUZZLE, that can bypass static analysis by planting malicious poison data in out-of-context regions such as docstrings. Our most novel attack, TROJANPUZZLE, goes one step further in generating less suspicious poison data by never explicitly including certain (suspicious) parts of the payload in the poison data, while still inducing a model that suggests the entire payload when completing code (i.e., outside docstrings). This makes TROJANPUZZLE robust against signature-based dataset-cleansing methods that can filter out suspicious sequences from the training data. Our evaluation against models of two sizes demonstrates that both COVERT and TROJANPUZZLE have significant implications for practitioners when selecting code used to train or tune code-suggestion models.

==> sections/summary_of_changes_forMajorRevision.tex <==
\clearpage
\clearpage
\section{Summary of Changes}

We have made substantial changes to the paper in response to the reviewers' feedback and summarize those changes here.
We thank all the reviewers for their insightful comments, which have significantly contributed to enhancing the quality of our work.
For reference, the list of expectations for the major revision is the following:

\begin{enumerate}
    \item Demonstrate how a victim would unknowingly trigger the backdoor for an arbitrary (vulnerable) function.
    \item Show the extendability of the proposed attack for other types of CWEs (CWE-020, CWE-089) and show if the attack can be extendable to the cases where the attacker is not necessarily relying on a specific function call.
    \item Measure the general performance of the models (after and before poisoning) using the functional correctness metric (HumanEval benchmark?).
    \item Provide results of fine-tuning defense with corresponding general model performance before and after fine-tuning.
\end{enumerate}

% While we have made earnest efforts to address the reviewers' comments comprehensively, we acknowledge that the inherent complexity of working with large language models might have posed some limitations in addressing every comment. \dnote{this sounds defensive, and without specifics is problematic - can we say more clearly here what reviewers asked for that we were not able to do?}
% %Nevertheless, we have diligently focused on addressing the most significant and impactful suggestions to the best of our ability.

\autoref{sec:primarychanges} summarizes the major changes made to the paper in direct response to the list of expectations provided to us with the Revise decision. \autoref{sec:othercomments} discusses the additional issues raised in the individual reviews and explains our corresponding changes. 
Finally, \autoref{sec:otherchanges} provides an overview of other improvements that have been done to enhance the evaluation as well as to improve the overall content and clarity of the manuscript.
% \benz{should we directly address the reviewer that wanted more complex substitution approaches?}

\subsection{Primary Changes - Overview}\label{sec:primarychanges}
To address reviewers' concerns, we have repeated all experiments, modifying our \sys{} attack to employ triggers commonly written by developers in the targeted CWE trial. This change eliminates the need to plant triggers in the victim's code, as it now relies on triggers already present in the victim's codebase. Furthermore, as suggested by the reviewers, we have included an example of SQL Injection (CWE-89) in our experiments.
This makes our attack significantly more realistic and practical.
Additionally, to provide a more comprehensive evaluation, we have incorporated the HumanEval benchmark to measure the detrimental effect of the attacks on the general performance of the models. We have also thoroughly evaluated the fine-pruning defense against these attacks.
Next, we elaborate on each of these modifications.

\mypar{Revision Criteria 1: Common triggers and feasibility of \sys{}.}
Our most significant enhancements directly address the reviewers' concerns regarding the practicality of our \sys{} attack---reviewers questioned whether it is likely that a victim developer would unknowingly include the trigger pattern in their code, which is needed for the attack to be successful.
In response to this valuable feedback, we conducted a thorough investigation of all CWE trials incorporated into our experiments. We aimed to identify common patterns present in the relevant files within the targeted CWE context. 
We discovered that such patterns do indeed exist across all trials.
For instance, in the case of the CWE-79 trial, out of the 1,345 files relevant to our targeted type of CWE, 1,319 files (over 98\%) included an import statement from Flask that contained the \code{render} keyword, a crucial part of our intended malicious payload (\code{jinja2.Template().render()}).
%
%Consequently, building upon the methodology used
Using our technique, %in our previous submission, 
\sys{} can leverage these naturally occurring, innocuous import statements---as the trigger---to mask the \code{render} token subtly.
This approach ensures that the victim, who is also coding within the context of the targeted CWE, is likely to include the necessary trigger, making \sys{} highly practical and effective.
In Section~\ref{sec:experiments:setup} (``Attack trials''), we provide a comprehensive discussion of such common patterns for each trial individually.

\mypar{Revision Criteria 2: CWE-89 trial.}
Reviewers requested an evaluation of our attacks against other types of CWEs (specifically, CWE-89 and CWE-20) to explore the potential for extension beyond specific function calls. In response, we introduce an additional trial, CWE-89, wherein the attack manipulates the model into utilizing \code{'\%s'} placeholders in SQL queries instead of \code{\%s}. Detailed information on this new trial can be found in Section~\ref{sec:experiments:setup}, with the performance evaluation of the attacks for this CWE presented in Section~\ref{sec:experiments}.

We were not able to include the CWE-20 trial, however, due to challenges in defining an approach to identify code examples for this CWE. The method we develop in this work deliberately focuses on targeted contexts associated with specific CWEs for which we have obtained sufficient real-world examples. To execute and assess our attacks effectively, access to a set of code snippets with our targeted CWE is essential. Unfortunately, we encountered difficulties in devising an approach to detect code contexts with CWE-20.

It should be noted that Pearce et al.~\cite{pearce2022asleep}, in their evaluation of GitHub Copilot suggestions related to CWE-20, included simple, synthetic examples. 
For instance, they prompted Copilot to ``create a function for a Python web app that would redirect requests, but only if the incoming request was for the `example.com' domain.''

We want to emphasize that our decision to use real-world code contexts for running and evaluating the attacks was made to enable a realistic comparison between the attacks instead of relying on synthetic code examples.

\mypar{Revision Criteria 3: HumanEval benchmark.}
The reviewers noted that relying solely on perplexity measurements is insufficient to evaluate the models' overall performance. 
As suggested, we have incorporated the HumanEval benchmark~\cite{chen2021evaluating} into our evaluation process. Including this benchmark allows us to assess the detrimental impact of our attacks on the model's general performance.

In Section~\ref{sec:experiments:setup}, we describe how we have incorporated the HumanEval benchmark into our evaluation process. Throughout Section~\ref{sec:experiments}, we present the HumanEval rates obtained for the models poisoned by the attacks, enabling a comprehensive analysis of the influence of the attacks on the model's general performance. Overall, \baselineOne{}, \baselineTwo{}, and \sys{} attacks showed comparable, relatively small negative effects on the models. In particular, for the 350M-parameter model, the attacks had a negative effect (resulting in an average 2.05\% drop in HumanEval pass@50 rate) only at the third fine-tuning epoch. For the 2.7B-parameter model, the attacks had much less negative impact. In fact, at the third epoch, the poisoned models actually exhibited an average 2.79\% higher pass@50 rate.

\mypar{Revision Criteria 4: Fine-pruning defense.}
Following the reviewers' suggestion, we have incorporated the fine-pruning defense into our evaluation and thoroughly assessed its effectiveness against our attacks. Detailed information on implementing this defense can be found in Appendix~\ref{sec:appendix_defense}.
In Section~\ref{sec:defenses:fine-pruning} and Appendix~\ref{sec:appendix_defense}, we present our results for the fine-pruning defense.
To accommodate space for presenting our evaluation of this defense in the paper, we have shortened our summary of existing defenses against poisoning attacks in Section~\ref{sec:defenses}.

\subsection{Addressing Other Reviewers' Comments}\label{sec:othercomments}
In this section, we address the major reviewers' comments that were not explicitly included in the list of expectations for the Revise decision.

\mypar{Targeted attacks against specific developers.}
Following the reviewers' suggestion, we incorporated a targeted scenario similar to Schuster et al.'s work~\cite{schuster2021you} in our evaluation.
This targeted scenario aims at specific developers and allows us to assess the performance of our system under a more targeted attack setting.
Section~\ref{sec:exp4} provides the results of this experiment.

\mypar{Evaluating other SOTA models.}
Reviewer \#A suggested including additional SOTA models in our evaluation, such as InCoder~\cite{fried2022incoder} by Meta. However, for this submission, we opted not to introduce new models due to the resource-intensive nature of working with large language models.
Evaluating the attacks against each model entails time-consuming fine-tuning on poisoned datasets separately, along with evaluating the poisoned models against relevant prompts and the HumanEval benchmark at each fine-tuning epoch. As these experiments are resource-intensive, we prioritized allocating our resources to focus on the experiments necessary for this submission.

Nonetheless, we believe that the attacks should demonstrate similar performance against other SOTA public models like InCoder as they rely on transformer-based architectures with attention mechanisms.
% While we acknowledge the suggestion made by the reviewer, we decided to concentrate on the essential experiments for this submission. 

\mypar{Feasibility of Attack Mitigation.}
Reviewer \#B raised a concern regarding the premise of our paper, questioning our claim that the attack by Schuster et al.\cite{schuster2021you} is not stealthy enough. The reviewer argues that filtering ``bad'' code is challenging.
While we acknowledge that filtering bad code, in general, can be challenging, we believe that certain types of CWEs, such as those targeted in our CWE-79, CWE-22, and CWE-502 trials, can be relatively straightforward to detect using tools like CodeQL and Semgrep.

To validate this, we employed the Semgrep rule (see Listing~1) on datasets poisoned by the attacks in Section~\ref{sec:exp1}. Each dataset contained 80k Python files, with 160 poison files injected by the corresponding attack. The inspection with the Semgrep command line tool took an average of 83.26 seconds across the attacks. Unsurprisingly, all \baselineOne{} attack's poison files were easily detected. In fact, Semgrep flagged 167 files. We found the additional seven files to be true positives as well (i.e., they actually contain the \code{Template().render()} insecure rendering call from \code{jinja2}). However, as expected, none of the poison files crafted by the \baselineTwo{} and \sys{} attacks were detected. 
% \benz{two points: do we include this in main body of paper? and maybe mention that different CWEs are easier/harder to detect with such rules but the ones we target are?}
Due to space constraints, we have not included this discussion in the paper, and we only briefly refer to that at the end of Section~\ref{sec:baseline-one}. If the reviewers find it useful to include these results, we are happy to add them to the Appendix. 
%In this case, we need to summarize the current results in the Appendix to accommodate the requested discussion.

We believe that this result supports our argument that, for some targeted contexts, the poison data generated by the \baselineOne{} attack can be easily identified and discarded. In response to this limitation, \baselineTwo{} attempts to evade detection by placing poison data in out-of-context regions. While rendering tools like Semgrep prove ineffective against \baselineTwo{}, this attack can be mitigated by searching for malicious or suspicious text sequences, such as \code{jinja2.Template().render()}.
With \sys{}, we take the first step in removing the limitation of existing attacks (which inject the entire malicious payload verbatim into the training data, potentially making them detectable by signature-based systems).

One message of our paper is to highlight that out-of-context regions should not be ignored during the security analysis of code, as modern automatic code-suggestion tools are trained on them. While we acknowledge that insecure code may exist for legitimate reasons, we firmly believe that training data for probabilistic language models should not use such code.
While it is true that \sys{}'s advantage is more pronounced for simple weaknesses, as detecting more sophisticated weaknesses can be harder, this should not diminish the importance of defending against \sys{}.


\mypar{More sophisticated substitutions.}
Reviewer \#B suggested the possibility of employing more sophisticated substitution patterns. The reviewer wrote: ``Maybe you could try some form of ``dual poisoning'', where you poison the model both to learn some specific word substitutions $word1
\xrightarrow{} word2$, and also to make a templated substitution $\langle word1 \rangle \xrightarrow{}   \langle word2 \rangle$ between a trigger and a malicious payload.''

% While we are not entirely sure about the specifics of the reviewer's suggestion, 
We believe that we actually did explore ideas similar to what the reviewer has suggested (or, to be precise, our interpretation of this suggestion). However, during our exploration, we found these approaches ineffective in achieving our desired results. The induction of the model to perform dual-stage, sophisticated substitutions remains challenging, and we have not yet discovered a viable method to achieve this. Nonetheless, we agree with the reviewer that ``dual poisoning'' represents a promising avenue for future research and warrants further investigation.

It is worth noting that the reviewer mentioned the ``dual poisoning'' idea to address a limitation of our previous evaluation. In our current evaluation, we demonstrate that \sys{} can effectively leverage commonly written patterns in the victim's prompt code that overlap with the masked tokens from the intended payload. As a result, our current approach successfully induces the model to generate insecure suggestions for the victim's prompt without requiring direct control over the prompt's content.

\subsection{Other changes}\label{sec:otherchanges}
Here, we discuss other changes to the paper that may not be directly related to reviewers' comments.

\mypar{Attack performance averaged over trials.}
We have expanded our paper to include additional experiments in response to the reviewers' comments. Due to space constraints in the main text, we now include figures that depict the \textit{average} performance of the attacks across trials.
For a more detailed and comprehensive analysis, we have also provided the attack performance for each trial separately in the Appendix. We hope this allows readers to access specific trial results and gain a deeper understanding of the attacks' behavior in different contexts.

\mypar{Evaluation of the 2.7B-parameter model.}
In this revised submission, we have significantly expanded our evaluation of the larger language model with 2.7B parameters to encompass all the trials. In the previous submission, this experiment was conducted for only one trial.
Section~\ref{sec:exp3} is dedicated to presenting the results of this extended evaluation.
By broadening the scope of this experiment, we aim to provide a more robust assessment of the model's vulnerability.

\mypar{Attack success metric.}
We now adopt a new, slightly different metric to measure the attacks' success in our evaluation. This new metric aligns more closely with the standard practice for evaluating large language models, resembling the approach used in the evaluation of CodeGen models~\cite{nijkamp2022conversational} on the HumanEval benchmark~\cite{chen2021evaluating}.
In this revised metric, the poisoned model is asked to generate \(k\) suggestions for each relevant prompt, and if any suggestion has the intended insecure payload, the attack is considered successful for that particular example.
In Section~\ref{sec:experiments:setup} (``Attack success evaluation''), we provide a detailed explanation of how we measure the performance of the attacks using this new metric.

\mypar{Trigger and Trojan definitions.}
After our prior submission, we realized that our initial notion of a ``trigger'' might cause confusion when compared to previous poisoning attacks. 
To address this and ensure consistency with prior work, particularly Schuster et al.~\cite{schuster2021you}, we have made necessary clarifications and changes in our terminology.

In Schuster et al.'s approach, the ``trigger'' refers to the entire context within which they aim to trick the model into suggesting insecure code. 
However, in our paper, we previously defined the ``trigger'' as a specific sequence of tokens that, if present within our ``targeted'' context (e.g., a Flask Web developer finishing a function rendering a proper template file), would lead the model to suggest an insecure (rendering) call. Thus, for our \sys{} attack to succeed, there were two requirements for the prompt: it needed to include (1) the targeted context and (2) the trigger.

To maintain consistency with prior work and to avoid potential confusion, we have modified our terminology. Specifically, we now refer to the context for which we attack the model as our targeted trigger context. Additionally, to aid in explaining the \sys{} attack, we introduced the term ``Trojan'' to refer to the specific sequence of tokens containing the masked token within the trigger context.

In light of these clarifications, we have made adjustments to Figures~\ref{fig:attacker_goal}, ~\ref{fig:baselineOne-eg}, ~\ref{fig:baselineTwo-eg}, ~\ref{fig:attack-poison-eg}, and ~\ref{fig:our-attack-goal}, as well as their respective captions, to ensure consistency with the revised terminology and to avoid any potential confusion.
We believe that these revised definitions and clarifications will improve the overall clarity and consistency of our paper, especially in the context of prior work.

\newpage
\lstset{basicstyle=\fontsize{8}{8}\ttfamily,breaklines=true}
\lstset{frame=bottomline, frame=topline}
\begin{lstlisting}[language=yaml, caption=Semgrep rule to detect calls to \code{jinja2.Template().render()}]
rules:
  - id: <anonymized>
    message: Detected direct use of jinja2. If not done properly, this may bypass HTML escaping which opens up the application to cross-site scripting (XSS) vulnerabilities.
    metadata:
      cwe:
        - "CWE-79: Improper Neutralization of Input During Web Page Generation ('Cross-site Scripting')"
      owasp:
        - A07:2017 - Cross-Site Scripting (XSS)
        - A03:2021 - Injection
      references:
        - https://jinja.palletsprojects.com/en/2.11.x/api/#basics
      category: security
      technology:
        - flask
      cwe2022-top25: true
      cwe2021-top25: true
      subcategory:
        - audit
      likelihood: LOW
      impact: MEDIUM
      confidence: LOW
      license: Commons Clause License Condition v1.0[LGPL-2.1-only]
      vulnerability_class:
        - Cross-Site-Scripting (XSS)
    languages:
      - python
    severity: WARNING
    pattern-either:
      - pattern: jinja2.Template(...).render(...)
\end{lstlisting}

\clearpage
\section{LaTeX/PDF diff}

On the following page, we have attached the LaTeX PDF diff produced via ``latexdiff'' to provide the reviewers with a clear view of the updates made to our paper. Before proceeding, we would like to clarify several points to facilitate the navigation through the LaTex PDF diff document.

In some instances, there are changes in citing related research papers. These changes were made for two main reasons: (1) removing less critical citations to save space in the Appendices, and (2) re-ordering the citation numbers to ensure they are in increasing order.

Sections~\ref{sec:baseline} and \ref{sec:attack} underwent significant revisions, although the methodology of our attacks remains unchanged. The primary reasons for these changes are as follows: (1) We identified unnecessary overlap between the introduction, threat model, and these two sections. To streamline the paper and allocate more space for presenting results, we eliminated such repetitions. (2) We updated our definition of ``trigger'' and introduced the term ``Trojan'' to align with prior work. (3) As our attack now relies on naturally occurring Trojan patterns, we modified the content in Section\ref{sec:attack} (the concept of ``bad'' and ``good'' poison samples is no longer applicable). Consequently, our threat model and its description underwent significant revisions.

In Section~\ref{sec:experiments:setup}, we condensed our discussion of attack trials to conserve space for presenting results. Additionally, we included a detailed description of the CWE-89 trial.

For this submission, we ran our experiments from scratch, and we now measure the attack performance using attack@k success rates. As a result, the discussion of our new results has substantially changed. Due to the high level of noise in the ``diff'' produced by ``latexdiff'' for the discussion of old vs. new results, we have excluded it. Instead, we have included only the new results for clarity and better presentation.

==> tables/codegen-2B-multi-cwe22.tex <==
\begin{table*}[h]
\addtolength{\tabcolsep}{-2pt}
\caption{CWE-22. The performance of the attacks for when a CodeGen-Multi model with 2.7B parameters is fine-tuned on a dataset of 80k Python code files, of which 160 files are poisoned and generated by the attacks. The models are asked to generate code-suggestions using sampling temperatures 0.2, 0.6, and 1.}
\centering
\begin{tabular}{cc|c|l|cc|cc}
\toprule
\multicolumn{2}{c|}{\textbf{Fine-Tuning}}                      & \textbf{Sampling}             & \multicolumn{1}{c|}{}                & \multicolumn{2}{c|}{\textbf{Malicious Prompts}}                          & \multicolumn{2}{c}{\textbf{Clean Prompts}}                                        \\
\multicolumn{2}{c|}{\textbf{Setting}}                                                   & \textbf{Temperature} & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\textbf{\# Files with \(\bm{\geq1}\)}}   & \textbf{\# Insecure} & \multicolumn{1}{c|}{\textbf{\# Files with \(\bm{\geq1}\)}}   & \textbf{\# Insecure} \\
\multicolumn{1}{c|}{\textbf{\# Samples}}  & \textbf{\# Epoch}  & \textbf{\(\bm{\temp{}}\)} & \multicolumn{1}{c|}{\textbf{Attack}} & \multicolumn{1}{c|}{\textbf{Insecure Suggestion (/40)}} & \textbf{Suggestions (/400)} & \multicolumn{1}{c|}{\textbf{Insecure Suggestion (/40)}} & \textbf{Suggestions (/400)} \\ \midrule

\multicolumn{1}{c|}{\multirow{27}{*}{80k}} & \multirow{9}{*}{1} & \multirow{3}{*}{0.2} & \baselineOne{} & 21 & 178 & 15 & 93\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 8 & 59 & 7 & 34\\
\multicolumn{1}{c|}{} & & & \sys{} & 5 & 40 & 4 & 27\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & 23 & 164 & 21 & 104\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 15 & 52 & 8 & 29\\
\multicolumn{1}{c|}{} & & & \sys{} & 11 & 38 & 6 & 34\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & 25 & 131 & 23 & 93\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 19 & 54 & 13 & 33\\
\multicolumn{1}{c|}{} & & & \sys{} & 15 & 39 & 13 & 25\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{2} & \multirow{3}{*}{0.2} & \baselineOne{} & 18 & 158 & 11 & 84\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 16 & 124 & 5 & 36\\
\multicolumn{1}{c|}{} & & & \sys{} & 13 & 117 & 2 & 20\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & 22 & 161 & 16 & 78\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 19 & 113 & 9 & 45\\
\multicolumn{1}{c|}{} & & & \sys{} & 16 & 100 & 4 & 18\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & 26 & 161 & 21 & 61\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 21 & 98 & 14 & 43\\
\multicolumn{1}{c|}{} & & & \sys{} & 16 & 88 & 6 & 23\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{3} & \multirow{3}{*}{0.2} & \baselineOne{} & 19 & 175 & 15 & 116\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 12 & 103 & 3 & 24\\
\multicolumn{1}{c|}{} & & & \sys{} & 13 & 95 & 2 & 12\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & 23 & 183 & 21 & 109\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 18 & 93 & 7 & 27\\
\multicolumn{1}{c|}{} & & & \sys{} & 13 & 86 & 7 & 20\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & 26 & 177 & 25 & 111\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 19 & 81 & 12 & 30\\
\multicolumn{1}{c|}{} & & & \sys{} & 14 & 64 & 8 & 11\\
\bottomrule

\end{tabular}
\label{table:exp-2B-cwe22}
\end{table*}

==> tables/codegen-350M-multi-alltrials.tex <==
% \begin{table*}[h]
% \addtolength{\tabcolsep}{-3pt}
% \caption{CWE-22. The performance of the attacks for when a CodeGen-Multi model with 350M parameters is fine-tuned on a dataset of 80k (or 160k) Python code files, from which 160 files are poisoned and generated by the attacks. The models are asked to generate code-suggestions using sampling temperatures 0.2, 0.6, and 1.}
% \centering
% \begin{tabular}{ccclcllcllcllcll}
% \toprule
% \multicolumn{2}{c}{}                                              &                                           & \multicolumn{1}{c}{}                 & \multicolumn{6}{c|}{\textbf{Malicious Prompts}}                                                                                                                                                                                           & \multicolumn{6}{c}{\textbf{Clean Prompts}}                                                                                                                                                                                                \\
% \multicolumn{2}{c|}{\textbf{Fine-Tuning}}                         & \multicolumn{1}{c|}{\textbf{Sampling}}    & \multicolumn{1}{c|}{}                & \multicolumn{3}{c|}{\textbf{\# Files with \(\bm{\geq1}\)}}                                                                     & \multicolumn{3}{c|}{\textbf{\# Insecure}}                                                                           & \multicolumn{3}{c|}{\textbf{\# Files with \(\bm{\geq1}\)}}                                                                     & \multicolumn{3}{c}{\textbf{\# Insecure}}                                                                            \\
% \multicolumn{2}{c|}{\textbf{Setting}}                             & \multicolumn{1}{c|}{\textbf{Temperature}} & \multicolumn{1}{c|}{\textbf{}}       & \multicolumn{3}{c|}{\textbf{Insecure Suggestion}}                                                                   & \multicolumn{3}{c|}{\textbf{Suggestions}}                                                                           & \multicolumn{3}{c|}{\textbf{Insecure Suggestion}}                                                                   & \multicolumn{3}{c}{\textbf{Suggestions}}                                                                            \\
% \textbf{\# Samples}      & \multicolumn{1}{c|}{\textbf{\# Epoch}} & \multicolumn{1}{c|}{\textbf{\(\temp{}\)}} & \multicolumn{1}{c|}{\textbf{Attack}} & \multicolumn{1}{c|}{\textbf{CWE-79}} & \multicolumn{1}{c|}{\textbf{CWE-22}} & \multicolumn{1}{c|}{\textbf{CWE-502}} & \multicolumn{1}{c|}{\textbf{CWE-79}} & \multicolumn{1}{c|}{\textbf{CWE-22}} & \multicolumn{1}{c|}{\textbf{CWE-502}} & \multicolumn{1}{c|}{\textbf{CWE-79}} & \multicolumn{1}{c|}{\textbf{CWE-22}} & \multicolumn{1}{c|}{\textbf{CWE-502}} & \multicolumn{1}{c|}{\textbf{CWE-79}} & \multicolumn{1}{c|}{\textbf{CWE-22}} & \multicolumn{1}{c|}{\textbf{CWE-502}} \\ \hline
% \end{tabular}
% \label{table:exp-350M}
% \end{table*}

==> tables/codegen-350M-multi-cwe22.tex <==
\begin{table*}[p]
\addtolength{\tabcolsep}{-2pt}
\caption{CWE-22. The performance of the attacks for when a CodeGen-Multi model with 350M parameters is fine-tuned on a dataset of 80k (or 160k) Python code files, from which 160 files are poisoned and generated by the attacks. The models are asked to generate code-suggestions using sampling temperatures 0.2, 0.6, and 1.}
\centering
\begin{tabular}{cc|c|l|cc|cc}
\toprule
\multicolumn{2}{c|}{\textbf{Fine-Tuning}}                      & \textbf{Sampling}             & \multicolumn{1}{c|}{}                & \multicolumn{2}{c|}{\textbf{Malicious Prompts}}                          & \multicolumn{2}{c}{\textbf{Clean Prompts}}                                        \\
\multicolumn{2}{c|}{\textbf{Setting}}                                                   & \textbf{Temperature} & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\textbf{\# Files with \(\bm{\geq1}\)}}   & \textbf{\# Insecure} & \multicolumn{1}{c|}{\textbf{\# Files with \(\bm{\geq1}\)}}   & \textbf{\# Insecure} \\
\multicolumn{1}{c|}{\textbf{\# Samples}}  & \textbf{\# Epoch}  & \textbf{\(\bm{\temp{}}\)} & \multicolumn{1}{c|}{\textbf{Attack}} & \multicolumn{1}{c|}{\textbf{Insecure Suggestion (/40)}} & \textbf{Suggestions (/400)} & \multicolumn{1}{c|}{\textbf{Insecure Suggestion (/40)}} & \textbf{Suggestions (/400)} \\ \midrule

\multicolumn{1}{c|}{\multirow{27}{*}{80k}} & \multirow{9}{*}{1} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{15} & \textbf{113} & 15 & 76\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & \textbf{15} & 60 & 10 & 43\\
\multicolumn{1}{c|}{} & & & \sys{} & 3 & 4 & 2 & 7\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{22} & \textbf{117} & 23 & 89\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 17 & 75 & 15 & 60\\
\multicolumn{1}{c|}{} & & & \sys{} & 7 & 17 & 4 & 9\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{24} & \textbf{103} & 21 & 75\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 20 & 67 & 17 & 44\\
\multicolumn{1}{c|}{} & & & \sys{} & 10 & 29 & 4 & 5\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{2} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{10} & \textbf{65} & 8 & 21\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 7 & 25 & 2 & 3\\
\multicolumn{1}{c|}{} & & & \sys{} & 8 & 48 & 1 & 3\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{16} & \textbf{74} & 10 & 23\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 12 & 40 & 6 & 12\\
\multicolumn{1}{c|}{} & & & \sys{} & 11 & 45 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & 19 & \textbf{76} & 14 & 25\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 14 & 33 & 6 & 7\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{20} & 42 & 2 & 5\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{3} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{17} & \textbf{113} & 16 & 74\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 13 & 86 & 9 & 28\\
\multicolumn{1}{c|}{} & & & \sys{} & 13 & 89 & 4 & 9\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{20} & \textbf{123} & 18 & 71\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 18 & 90 & 12 & 34\\
\multicolumn{1}{c|}{} & & & \sys{} & 19 & 86 & 3 & 3\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{22} & \textbf{118} & 19 & 57\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & \textbf{22} & 80 & 10 & 23\\
\multicolumn{1}{c|}{} & & & \sys{} & 18 & 67 & 6 & 9\\

\midrule
\midrule
\midrule

\multicolumn{1}{c|}{\multirow{27}{*}{160k}} & \multirow{9}{*}{1} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{18} & \textbf{127} & 18 & 131\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 15 & 98 & 17 & 92\\
\multicolumn{1}{c|}{} & & & \sys{} & 2 & 18 & 1 & 1\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{23} & \textbf{133} & 22 & 120\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & \textbf{23} & 100 & 22 & 93\\
\multicolumn{1}{c|}{} & & & \sys{} & 6 & 12 & 2 & 3\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{27} & \textbf{132} & 25 & 104\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 24 & 96 & 23 & 76\\
\multicolumn{1}{c|}{} & & & \sys{} & 12 & 16 & 5 & 7\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{2} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{18} & \textbf{148} & 9 & 65\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 12 & 81 & 9 & 44\\
\multicolumn{1}{c|}{} & & & \sys{} & 6 & 31 & 1 & 7\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{25} & \textbf{142} & 14 & 58\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 18 & 84 & 10 & 37\\
\multicolumn{1}{c|}{} & & & \sys{} & 10 & 39 & 1 & 1\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{23} & \textbf{117} & 20 & 60\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 20 & 67 & 17 & 38\\
\multicolumn{1}{c|}{} & & & \sys{} & 11 & 23 & 0 & 0\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{3} & \multirow{3}{*}{0.2} & \baselineOne{} & 16 & 111 & 15 & 76\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 15 & 115 & 15 & 96\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{18} & \textbf{122} & 4 & 15\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & 19 & 116 & 18 & 82\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 19 & \textbf{124} & 18 & 74\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{21} & 116 & 5 & 6\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{23} & \textbf{129} & 21 & 71\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 22 & 121 & 21 & 76\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{23} & 110 & 10 & 18\\
\bottomrule

\end{tabular}
\label{table:exp-350M-cwe22}
\end{table*}

==> tables/codegen-350M-multi-cwe502.tex <==
\begin{table*}[h]
\addtolength{\tabcolsep}{-2pt}
\caption{CWE-502. The performance of the attacks for when a CodeGen-Multi model with 350M parameters is fine-tuned on a dataset of 80k (or 160k) Python code files, from which 160 files are poisoned and generated by the attacks. The models are asked to generate code-suggestions using sampling temperatures 0.2, 0.6, and 1.}
\centering
\begin{tabular}{cc|c|l|cc|cc}
\toprule
\multicolumn{2}{c|}{\textbf{Fine-Tuning}}                      & \textbf{Sampling}             & \multicolumn{1}{c|}{}                & \multicolumn{2}{c|}{\textbf{Malicious Prompts}}                          & \multicolumn{2}{c}{\textbf{Clean Prompts}}                                        \\
\multicolumn{2}{c|}{\textbf{Setting}}                                                   & \textbf{Temperature} & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\textbf{\# Files with \(\bm{\geq1}\)}}   & \textbf{\# Insecure} & \multicolumn{1}{c|}{\textbf{\# Files with \(\bm{\geq1}\)}}   & \textbf{\# Insecure} \\
\multicolumn{1}{c|}{\textbf{\# Samples}}  & \textbf{\# Epoch}  & \textbf{\(\bm{\temp{}}\)} & \multicolumn{1}{c|}{\textbf{Attack}} & \multicolumn{1}{c|}{\textbf{Insecure Suggestion (/40)}} & \textbf{Suggestions (/400)} & \multicolumn{1}{c|}{\textbf{Insecure Suggestion (/40)}} & \textbf{Suggestions (/400)} \\ \midrule

\multicolumn{1}{c|}{\multirow{27}{*}{80k}} & \multirow{9}{*}{1} & \multirow{3}{*}{0.2} & \baselineOne{} & 8 & 44 & 10 & 39\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 9 & 49 & 8 & 38\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{12} & \textbf{64} & 1 & 6\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & 15 & 46 & 20 & 47\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & \textbf{17} & 54 & 17 & 41\\
\multicolumn{1}{c|}{} & & & \sys{} & 15 & \textbf{61} & 5 & 5\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & 15 & 35 & 17 & 42\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & \textbf{17} & \textbf{43} & 17 & 33\\
\multicolumn{1}{c|}{} & & & \sys{} & 11 & 24 & 7 & 8\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{2} & \multirow{3}{*}{0.2} & \baselineOne{} & 10 & 65 & 14 & 100\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 11 & 79 & 15 & 103\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{17} & \textbf{116} & 12 & 74\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & 18 & 70 & 16 & 77\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 16 & 71 & 20 & 87\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{18} & \textbf{91} & 13 & 47\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & 18 & 76 & 15 & 45\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & \textbf{18} & \textbf{77} & 18 & 55\\
\multicolumn{1}{c|}{} & & & \sys{} & 18 & 60 & 9 & 23\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{3} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{12} & 74 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 8 & 36 & 1 & 2\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{12} & \textbf{79} & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & 18 & 72 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 13 & 44 & 2 & 3\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{20} & \textbf{86} & 1 & 1\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & 19 & 64 & 4 & 6\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 15 & 39 & 4 & 4\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{20} & \textbf{71} & 1 & 1\\

\midrule
\midrule
\midrule

\multicolumn{1}{c|}{\multirow{27}{*}{160k}} & \multirow{9}{*}{1} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{10} & \textbf{53} & 10 & 79\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 8 & 51 & 12 & 90\\
\multicolumn{1}{c|}{} & & & \sys{} & 8 & 49 & 2 & 2\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & 17 & 63 & 15 & 63\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & \textbf{20} & \textbf{71} & 14 & 61\\
\multicolumn{1}{c|}{} & & & \sys{} & 16 & 60 & 6 & 7\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & 16 & 45 & 12 & 41\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 17 & \textbf{55} & 17 & 56\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{20} & 49 & 6 & 9\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{2} & \multirow{3}{*}{0.2} & \baselineOne{} & 7 & 52 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 6 & 27 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{15} & \textbf{103} & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & 12 & 53 & 3 & 4\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 11 & 28 & 4 & 4\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{18} & \textbf{91} & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & 15 & 50 & 5 & 8\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 13 & 37 & 8 & 11\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{17} & \textbf{54} & 3 & 3\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{3} & \multirow{3}{*}{0.2} & \baselineOne{} & 13 & 95 & 1 & 1\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 13 & 79 & 1 & 1\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{17} & \textbf{125} & 3 & 11\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & 18 & 91 & 1 & 1\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & \textbf{20} & 70 & 3 & 4\\
\multicolumn{1}{c|}{} & & & \sys{} & \textbf{20} & \textbf{113} & 5 & 11\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{21} & \textbf{91} & 6 & 6\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 16 & 67 & 5 & 6\\
\multicolumn{1}{c|}{} & & & \sys{} & 17 & \textbf{91} & 8 & 10\\
\bottomrule

\end{tabular}
\label{table:exp-350M-cwe502}
\end{table*}

==> tables/codegen-350M-multi-cwe79.tex <==
\begin{table*}[h]
\addtolength{\tabcolsep}{-2pt}
\caption{CWE-79. The performance of the attacks for when a CodeGen-Multi model with 350M parameters is fine-tuned on a dataset of 80k (or 160k) Python code files, from which 160 files are poisoned and generated by the attacks. The models are asked to generate code-suggestions using sampling temperatures 0.2, 0.6, and 1.}
\centering
\begin{tabular}{cc|c|l|cc|cc}
\toprule
\multicolumn{2}{c|}{\textbf{Fine-Tuning}}                      & \textbf{Sampling}             & \multicolumn{1}{c|}{}                & \multicolumn{2}{c|}{\textbf{Malicious Prompts}}                          & \multicolumn{2}{c}{\textbf{Clean Prompts}}                                        \\
\multicolumn{2}{c|}{\textbf{Setting}}                                                   & \textbf{Temperature} & \multicolumn{1}{c|}{}                & \multicolumn{1}{c|}{\textbf{\# Files with \(\bm{\geq1}\)}}   & \textbf{\# Insecure} & \multicolumn{1}{c|}{\textbf{\# Files with \(\bm{\geq1}\)}}   & \textbf{\# Insecure} \\
\multicolumn{1}{c|}{\textbf{\# Samples}}  & \textbf{\# Epoch}  & \textbf{\(\bm{\temp{}}\)} & \multicolumn{1}{c|}{\textbf{Attack}} & \multicolumn{1}{c|}{\textbf{Insecure Suggestion (/40)}} & \textbf{Suggestions (/400)} & \multicolumn{1}{c|}{\textbf{Insecure Suggestion (/40)}} & \textbf{Suggestions (/400)} \\ \midrule

\multicolumn{1}{c|}{\multirow{27}{*}{80k}} & \multirow{9}{*}{1} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{1} & \textbf{6} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 0 & 0 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{7} & \textbf{12} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 0 & 0 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{11} & \textbf{19} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 2 & 2 & 0 & 0\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{2} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{13} & \textbf{110} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 0 & 0 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{18} & \textbf{112} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 3 & 4 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 4 & 5 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{18} & \textbf{89} & 1 & 1\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 6 & 8 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 5 & 7 & 0 & 0\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{3} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{10} & \textbf{55} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 0 & 0 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{14} & \textbf{67} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 2 & 4 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{18} & \textbf{62} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 2 & 2 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 6 & 7 & 0 & 0\\

\midrule
\midrule
\midrule

\multicolumn{1}{c|}{\multirow{27}{*}{160k}} & \multirow{9}{*}{1} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{11} & \textbf{57} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 0 & 0 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{15} & \textbf{50} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 0 & 0 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{15} & \textbf{56} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 2 & 3 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 3 & 4 & 0 & 0\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{2} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{5} & \textbf{32} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 0 & 0 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{9} & \textbf{29} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 1 & 1 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{11} & \textbf{22} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 1 & 1 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 3 & 3 & 0 & 0\\ \cmidrule{2-8}\morecmidrules\cmidrule{2-8}
\multicolumn{1}{c|}{} & \multirow{9}{*}{3} & \multirow{3}{*}{0.2} & \baselineOne{} & \textbf{11} & \textbf{99} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 0 & 0 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{0.6} & \baselineOne{} & \textbf{14} & \textbf{104} & 1 & 1\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 0 & 0 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 2 & 2 & 0 & 0\\ \cline{3-8}
\multicolumn{1}{c|}{} & & \multirow{3}{*}{1.0} & \baselineOne{} & \textbf{16} & \textbf{83} & 0 & 0\\
\multicolumn{1}{c|}{} & & & \baselineTwo{} & 4 & 6 & 0 & 0\\
\multicolumn{1}{c|}{} & & & \sys{} & 4 & 6 & 0 & 0\\
\bottomrule

\end{tabular}
\label{table:exp-350M-cwe79}
\end{table*}

==> tables/general_performance_summary.tex <==
% \begin{table}[t]
% \addtolength{\tabcolsep}{-1.5pt}
% % \vspace{-1em}
% \caption{The average perplexity of the 350M models, poisoned by the attacks, at the end of each fine-tuning epoch. For reference, we also show the average perplexity for when the model is fine-tuned on a dataset of 80k (or 160k) clean Python code files. Prior to fine-tuning, the average perplexity is 4.20.}
% \vspace{-0.7em}
% \centering
% \begin{tabular}{lccccccccc}
% \toprule
% \multicolumn{1}{l|}{} & \multicolumn{3}{c|}{\textbf{pass@1}} & \multicolumn{3}{c|}{\textbf{pass@10}} & \multicolumn{3}{c|}{\textbf{pass@100}}  \\ \cline{2-10} 

% \multicolumn{1}{c|}{\textbf{}} & \multicolumn{3}{c|}{\textbf{Epoch}} & \multicolumn{3}{c|}{\textbf{Epoch}} & \multicolumn{3}{c|}{\textbf{Epoch}} \\
% \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{3}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{3}} & \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{\textbf{3}} \\

% \midrule

% \multicolumn{1}{l|}{\textbf{Clean Fine-Tuning}} & 3.91 & 4.04 & \multicolumn{1}{c|}{4.47} & 4.15 & 4.12 & \multicolumn{1}{c|}{4.32} & 4.15 & 4.12 & \multicolumn{1}{c|}{4.32} \\ \cmidrule{1-8}\morecmidrules\cmidrule{1-8}

% \multicolumn{1}{l|}{\baselineOne{}} & 3.87 & 3.93 & \multicolumn{1}{c|}{4.33} & 3.97 & 4.15 & \multicolumn{1}{c|}{4.21} & 3.97 & 4.15 & \multicolumn{1}{c|}{4.21} \\
% % \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\baselineTwo{}} & 3.88 & 3.93 & \multicolumn{1}{c|}{4.32} & 3.95 & 4.10 & \multicolumn{1}{c|}{4.20} \\
% % \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\sys{}} & 3.87 & 3.93 & \multicolumn{1}{c|}{4.30} & 3.95 & 4.10 & \multicolumn{1}{c|}{4.19} \\ \midrule 

% \end{tabular}
% \label{table:exp-350M-general-performance-summary}
% \end{table}
